Physics-Based Adversarial Attack on Near-Infrared Human Detector for Nighttime Surveillance Camera Systems

Many surveillance cameras switch between daytime and nighttime modes based on illuminance levels. During the day, the camera records ordinary RGB images through an enabled IR-cut filter. At night, the filter is disabled to capture near-infrared (NIR) light emitted from NIR LEDs typically mounted around the lens. While RGB-based AI algorithm vulnerabilities have been widely reported, the vulnerabilities of NIR-based AI have rarely been investigated. In this paper, we identify fundamental vulnerabilities in NIR-based image understanding caused by color and texture loss due to the intrinsic characteristics of clothes' reflectance and cameras' spectral sensitivity in the NIR range. We further show that the nearly co-located configuration of illuminants and cameras in existing surveillance systems facilitates concealing and fully passive attacks in the physical world. Specifically, we demonstrate how retro-reflective and insulation plastic tapes can manipulate the intensity distribution of NIR images. We showcase an attack on the YOLO-based human detector using binary patterns designed in the digital space (via black-box query and searching) and then physically realized using tapes pasted onto clothes. Our attack highlights significant reliability concerns for nighttime surveillance systems, which are intended to enhance security. Codes Available: https://github.com/MyNiuuu/AdvNIR

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> samples/camera-ready.tex <==
%%
%% This is file `sample-sigconf.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% samples.dtx  (with options: `sigconf')
%% 
%% IMPORTANT NOTICE:
%% 
%% For the copyright see the source file.
%% 
%% Any modified versions of this file must be renamed
%% with new filenames distinct from sample-sigconf.tex.
%% 
%% For distribution of the original source see the terms
%% for copying and modification in the file samples.dtx.
%% 
%% This generated file may be distributed as long as the
%% original source files, as listed above, are part of the
%% same distribution. (The sources need not necessarily be
%% in the same archive or directory.)
%%
%%
%% Commands for TeXCount
%TC:macro \cite [option:text,text]
%TC:macro \citep [option:text,text]
%TC:macro \citet [option:text,text]
%TC:envir table 0 1
%TC:envir table* 0 1
%TC:envir tabular [ignore] word
%TC:envir displaymath 0 word
%TC:envir math 0 word
%TC:envir comment 0 0
%%
%%
%% The first command in your LaTeX source must be the \documentclass
%% command.
%%
%% For submission and review of your manuscript please change the
%% command to \documentclass[manuscript, screen, review]{acmart}.
%%
%% When submitting camera ready or to TAPS, please change the command
%% to \documentclass[sigconf]{acmart} or whichever template is required
%% for your publication.
%%
%%
% \documentclass[sigconf]{acmart}
% \documentclass[manuscript, screen, review]{acmart}.

\usepackage{booktabs}
\usepackage{caption}
\usepackage{multirow}

\newcommand\etal{\textit{et al.}}
\newcommand\eg{\textit{e.g.}}
\newcommand\ie{\textit{i.e.}}
\newcommand\etc{\textit{etc.}}


%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    Bib\TeX}}}


% \setcopyright{acmcopyright}
% \copyrightyear{2023}
% \acmYear{2023}
% \acmDOI{3581783.3612082}
% \acmConference[ACM MM'23]{ACM MM'23: ACM International Conference on Multimedia}{Oct.29--Nov.3, 2023}{Ottawa, Canada}
% \acmPrice{15.00}
% \acmISBN{978-1-4503-XXXX-X/18/06}


\copyrightyear{2023} 
\acmYear{2023} 
\setcopyright{acmlicensed}\acmConference[MM '23]{Proceedings of the 31st ACM International Conference on Multimedia}{October 29-November 3, 2023}{Ottawa, ON, Canada}
\acmBooktitle{Proceedings of the 31st ACM International Conference on Multimedia (MM '23), October 29-November 3, 2023, Ottawa, ON, Canada}
\acmPrice{15.00}
\acmDOI{10.1145/3581783.3612082}
\acmISBN{979-8-4007-0108-5/23/10}

%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% For managing citations, it is recommended to use bibliography
%% files in BibTeX format.
%%
%% You can then either use BibTeX with the ACM-Reference-Format style,
%% or BibLaTeX with the acmnumeric or acmauthoryear sytles, that include
%% support for advanced citation of software artefact from the
%% biblatex-software package, also separately available on CTAN.
%%
%% Look at the sample-*-biblatex.tex files for templates showcasing
%% the biblatex styles.
%%

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}


%%
%% end of the preamble, start of the body of the document source.
\begin{document}

%%
%% The "title" command has an optional parameter,
%% allowing the author to define a "short title" to be used in page headers.
\title{Physics-Based Adversarial Attack on Near-Infrared Human Detector for Nighttime Surveillance Camera Systems}

%%
%% The "author" command and its associated commands are used to define
%% the authors and their affiliations.
%% Of note is the shared affiliation of the first two authors, and the
%% "authornote" and "authornotemark" commands
%% used to denote shared contribution to the research.
\author{Muyao Niu}
\email{muyao.niu@gmail.com}
\affiliation{%
  \institution{The University of Tokyo}
  \country{Tokyo, Japan}
}

\author{Zhuoxiao Li}
\email{lizhuoxiao@g.ecc.u-tokyo.ac.jp}
\affiliation{%
  \institution{The University of Tokyo}
  \country{Tokyo, Japan}
}

\author{Yifan Zhan}
\email{zhan-yifan@g.ecc.u-tokyo.ac.jp}
\affiliation{%
  \institution{The University of Tokyo}
  \country{Tokyo, Japan}
}

\author{Huy H. Nguyen}
\email{nhhuy@nii.ac.jp}
\affiliation{%
  \institution{National Institute of Informatics}
  \country{Tokyo, Japan}
}

\author{Isao Echizen}
\email{iechizen@nii.ac.jp}
\affiliation{%
  \institution{National Institute of Informatics}
  \country{Tokyo, Japan}
}

\author{Yinqiang Zheng}
\authornote{Corresponding author.}
\email{yqzheng@ai.u-tokyo.ac.jp}
\affiliation{%
  \institution{The University of Tokyo}
  \country{Tokyo, Japan}
}

%%
%% By default, the full list of authors will be used in the page
%% headers. Often, this list is too long, and will overlap
%% other information printed in the page headers. This command allows
%% the author to define a more concise list
%% of authors' names for this purpose.
\renewcommand{\shortauthors}{Muyao Niu et al.}
%% No italics and no comma
%% If needed use a foot or author note to identify equal contribution

%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
  Many surveillance cameras switch between daytime and nighttime modes based on illuminance levels. During the day, the camera records ordinary RGB images through an enabled IR-cut filter. At night, the filter is disabled to capture near-infrared (NIR) light emitted from NIR LEDs typically mounted around the lens. While the vulnerabilities of RGB-based AI algorithms have been widely reported, those of NIR-based AI have rarely been investigated. In this paper, we identify fundamental vulnerabilities in NIR-based image understanding caused by color and texture loss due to the intrinsic characteristics of clothes' reflectance and cameras' spectral sensitivity in the NIR range. We further show that the nearly co-located configuration of illuminants and cameras in existing surveillance systems facilitates concealing and fully passive attacks in the physical world. Specifically, we demonstrate how retro-reflective and insulation plastic tapes can manipulate the intensity distribution of NIR images. We showcase an attack on the YOLO-based human detector using binary patterns designed in the digital space (via black-box query and searching) and then physically realized using tapes pasted onto clothes. Our attack highlights significant reliability concerns about nighttime surveillance systems, which are intended to enhance security. Codes Available: \url{https://github.com/MyNiuuu/AdvNIR}.
\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
   <concept>
       <concept_id>10002978.10003006</concept_id>
       <concept_desc>Security and privacy~Systems security</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
   <concept>
       <concept_id>10010147.10010178.10010224</concept_id>
       <concept_desc>Computing methodologies~Computer vision</concept_desc>
       <concept_significance>300</concept_significance>
       </concept>
 </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Security and privacy~Systems security}
\ccsdesc[300]{Computing methodologies~Computer vision}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Near-Infrared; Physical Adversarial Attack; Surveillance Systems}
%% A "teaser" image appears between the author and affiliation
%% information and the body of the document, and typically spans the
%% page.
% \begin{teaserfigure}
%   \includegraphics[width=\textwidth]{sampleteaser}
%   \caption{Seattle Mariners at Spring Training, 2010.}
%   \Description{Enjoying the baseball game from the third-base
%   seats. Ichiro Suzuki preparing to bat.}
%   \label{fig:teaser}
% \end{teaserfigure}

% \received{20 February 2007}
% \received[revised]{12 March 2009}
% \received[accepted]{5 June 2009}

%%
%% This command processes the author and affiliation and title
%% information and builds the first part of the formatted document.
\maketitle



\vspace{-2mm}

\section{Introduction}
% Surveillance camera systems have been widely installed for security purposes. Such systems can capture ordinary RGB images in the daytime, and the infrared component in daylight is filtered out by an IR-cut filter. In low-light environments such as midnight, it is difficult to obtain clear visible images due to limited camera sensitivity. The industry practice to solve this problem is to introduce near-infrared (NIR) LEDs for auxiliary illumination, which are mounted around the camera lens to save installation space (Fig.~\ref{fig:colocated}). The central wavelength of such NIR LEDs is usually around 850nm, which is covered by the spectral response range of silicon-based image sensors. NIR light at this wavelength is invisible to human eyes and is believed to be critical in reducing light pollution and hiding surveillance coverage. 

Surveillance camera systems are widely deployed for security purposes, capturing ordinary RGB images during the daytime while filtering out the infrared component with an IR-cut filter. However, in extremely low-light conditions such as midnight, clear visible images are difficult to obtain due to limited camera sensitivity. To address this, NIR LEDs are often utilized for auxiliary illumination.
% , mounted around the camera lens to save installation space and prevent occlusion
The central wavelength of these NIR LEDs is typically around 850nm, falling within the spectral response range of silicon-based image sensors. This NIR light is invisible to human eyes and helps to reduce light pollution while concealing surveillance coverage.

With the rapid development of deep learning-based visual AI, surveillance camera systems are becoming more intelligent, with advanced functionalities of human detection~\cite{redmon2016you,carion2020end}, face recognition~\cite{wen2016discriminative,schroff2015facenet}, \etc. The vulnerability of RGB-based vision has also been extensively studied, and countermeasures to protect them from attack have been proposed~\cite{hu2022adversarial,duan2021learning,huuu2022adversarial,suryanto2022dta,wang2022fca,tan2021legitimate}. 
% A surprising fact is that the potential vulnerabilities of NIR-based vision have never been reported in the literature, given its wide application scenarios in security fields such as surveillance cameras. 
% However, the potential vulnerabilities of NIR-based vision have never been reported in the literature. Given its wide application scenarios in security fields (\eg, surveillance cameras), these vulnerabilities may leave a window for attackers to exploit, causing great security issues. 

However, the potential vulnerabilities of NIR-based vision have rarely been explored. Although there have been attempts to use electronic devices worn on the face that emit near-infrared lights to hide human faces from cameras~\cite{yamada2013privacy,yamada2012use}, the potential vulnerabilities of NIR-based human body detectors have never been reported in existing studies. Given its wide application scenarios in security fields (\eg, surveillance cameras), these vulnerabilities may leave a window for attackers to exploit, causing great security issues. 

% In this paper, we bring this critical concern to the community and warn of the potential risks of relying on NIR-based AI in existing surveillance systems. By considering the imaging principle of NIR nighttime surveillance camera systems and the installation method of auxiliary lighting, several inherent vulnerabilities make NIR-based AI more brittle and less robust compared to RGB-based AI.

In this paper, we bring this critical concern to the community and warn of the potential risks of using AI algorithms in the NIR domain~\cite{redmon2016you,wu2017rgb,zhang2022fmcnet} for existing surveillance systems. By considering the imaging principle of NIR nighttime surveillance camera systems and the installation method of auxiliary lighting, several inherent vulnerabilities make NIR-based AI more brittle and less robust compared to RGB-based AI.


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/colorloss.pdf}
\setlength{\abovecaptionskip}{-4mm}
\caption{Illustration for color loss in NIR. Up: Camera Spectral Sensitivities of three different color cameras. Down: RGB images (a) and NIR images (b) for the same scene.}
\label{fig:colorloss}
\vspace{-6mm}
\end{figure}


Specifically, compared to visible illuminations, the NIR LED illumination around 850nm has the disadvantage that the color and texture of scene objects captured by the camera tend to disappear (Fig.~\ref{fig:colorloss}),
% (Figure~\ref{fig:page1}(d))
and this phenomenon particularly happens on textures of dyed fabrics such as human clothing~\cite{wu2020learn,liu2022optimal}. The reason lies in the fundamental imaging principle in the NIR range, which can be divided into two aspects. First, the spectral sensitivities of the three color filters of the silicon camera tend to overlap with each other in the NIR region, so monochromatic images can be acquired (Fig.~\ref{fig:colorloss}),
% (Figure~\ref{fig:page1}(b)(d))
though the sensor itself is trichromatic and the scene has brilliant colors. Second, the reflectance spectra of different materials also tend to coincide, resulting in severe texture loss. As a result, the intensity variation of NIR images is very limited, and the robustness of AI models trained on such data tends to be unstable. This implies the immediate vulnerability of AI models when the intensity distribution of the input image is somehow altered.

Regarding how to easily manipulate the intensity distribution in the physical world, we further recognize an intrinsic limitation of the geometric location of the auxiliary illuminant and the camera. To save installation space and reduce occlusion, LEDs are usually mounted around the lens (Fig.~\ref{fig:colocated}), which leads to a nearly co-located geometry setup. Given such a setting, the scene surface perpendicular to the viewing/lighting direction will lead to saturation when encountering certain materials. 

%when the direction of the light beam emitted from the LED matches the direction of the light beam entering the lens. As a result, the camera's auto-exposure function is activated to reduce the saturation effect and other image areas are likely to be darkened. By utilizing this feature of surveillance camera systems, we believe that it is possible to easily manipulate the luminance distribution of images captured by surveillance cameras.

In reality, we propose to use retro-reflective tape, which by design has a micro surface perpendicular to the viewing/lighting direction, irrespective of the geometric shape of the tape. This can be used to brighten an image area when needed. On the other hand, black plastic tapes (e.g., electrical insulating tape) have low NIR reflectance, allowing to reduce the intensity of an image area. Since retro-reflective tape's visible color (to human eyes) is independent of its reflectivity in the NIR range, we can use different color combinations to make the physical attacker appear natural to human eyes, further improving its stealthiness.

Based on the aforementioned vulnerabilities of NIR and the intensity manipulation via tapes with different materials, we showcase an attack instance on the YOLO-based human detector by first designing binary patterns in the digital space via black-box query and searching, neither requiring knowing the model parameters nor using any gradient-based optimization techniques. We leverage the 3D human models and renderer during the design process to consider real-world physical attributes. As a result, the designed pattern can be physically realized with appropriate tapes pasted onto clothes whose attack ability has been verified. Since retro-reflective tapes and insulation tapes are easily available at very low prices and the cost to make a physical attacker is extremely low, the proposed method will pose tremendous reliability concerns on NIR-based AI, widely introduced in nighttime surveillance systems for security and convenience. 

The contribution of this work can be summarized as follows:
\begin{itemize}
    \item We disclose the shortage of intensity variation in the NIR domain and analyze its physical mechanism from the perspective of camera spectral response and reflectance of dyed cloth, which finally leads to fundamental vulnerabilities of AI models on such images.
    \item We propose a fully passive yet effective method to manipulate the intensity distribution of NIR images captured by a co-located camera/illuminant system, mainly grounded on the well-known principle of retro-reflective materials. 
    \item We show an instance of how to attack the deep-learning based human detector in the blackbox style. Based on the principle of retro-reflective materials, the attacker is designed in a 3D-aware manner by introducing the 3D human models and rendering techniques in the digital space and can be easily implemented in the physical space with superior generalization abilities.
\end{itemize}




\section{Related Works}


\noindent \textbf{Physical Adversarial Attacks.} The RGB-based vision models grounded on deep learning are shown to be vulnerable to attacks, and various attacking and protection methods
% , either in the blackbox style or the whitebox style, 
have been extensively studied
% . We refer readers to those excellent review papers for more information
~\cite{moosavi2017universal,dong2018boosting,goodfellow2014explaining,madry2017towards,athalye2018synthesizing,carlini2017towards}. Instead of attacking in the digital space, more recent researches have tried to find effective attackers that can be physically realized~\cite{zhong2022shadows,zolfi2021translucent,jan2019connecting,eykholt2018robust,duan2020adversarial,duan2021adversarial,liu2019perceptual,liu2020bias,Zolfi_2021_CVPR}. 
% These attack methods can be divided into Whitebox attacks and Blackbox attacks
Among these methods, whitebox attacks~\cite{wu2020making,xu2020adversarial,tan2021legitimate,hu2021naturalistic,xingxing2023physically} possess knowledge of the model, including its structure, parameters, \etc. Consequently, these attacks are relatively straightforward to implement,
% The attacker uses the available information to identify the model's vulnerable feature space and adapt the attack method based on the defense technique and model parameters. 
and various physical attackers have been proposed~\cite{wu2020making,xu2020adversarial,tan2021legitimate,hu2021naturalistic}. On the other hand, blackbox attacks~\cite{zhong2022shadows,wei2022hotcold,diao2021basar,li2021adversarial,wei2020heuristic} involve situations where the attacker has no access to the structure and parameters of the target model. 
% Instead, the attacker can only interact with the model to obtain its predictions for particular samples. 
% Zhong \etal~\cite{zhong2022shadows} proposed a blackbox attack via the very common natural phenomenon—shadow. 
In this paper, we exploit the blackbox setting which has wider application scenarios since it does not need to know the structure and parameters of the target model.



% The patch-based adversarial attack methods aim to fool DNNs with elaborate patches and combinations. These models usually replace a localized region of the threat image with simple patch combinations, which enjoy high effectiveness and easy realization, thus has been frequently applied to real-world physical attacks~\cite{liu2019perceptual,liu2020bias,Zolfi_2021_CVPR} on state-of-the-art DNN-based methods. Wu~\etal~\cite{wu2020making} and Xu~\etal~\cite{xu2020adversarial} used physically printed posters and wearable clothes to realize patch-based attacks, \eg, adversarial T-shirt with designed attack patterns. However, these designed patterns are usually not stealthy enough due to its unnatural patterns. To address this problem, several works are proposed to generate cartoon-like patches that look more natural~\cite{tan2021legitimate,hu2021naturalistic}. We also follow this idea of designing natural patterns to improve stealthiness, and an important advantage of our NIR-based attack is that the visible color (to human eyes) will not affect the performance of attack in the NIR range. 


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/camera.pdf}
\setlength{\abovecaptionskip}{-2mm}
\caption{Co-located setup of surveillance camera systems.}
\label{fig:colocated}
\vspace{-6mm}
\end{figure}



\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{pictures/textureloss.pdf}
\setlength{\abovecaptionskip}{-4mm}
\caption{Illustration for texture loss in NIR. (a) RGB images with IR-cut filter, (b) NIR images through $>$ 700nm long-pass filter, (c) NIR images through 850nm band-pass filter with a full width at half magnitude (FWHM) of 40nm, whose spectral response is very close to the spectral distribution of 850nm LEDs. All images are captured with the same trichromatic camera, with its IR-cut filter removed when needed (b,c). We can see that, although the clothes have rich color and texture in the visible range, they tend to disappear, especially in the narrow spectral range covered by 850nm LEDs.}
\label{fig:textureloss}
\vspace{-4mm}
\end{figure*}


\noindent \textbf{Adversarial Attacks beyond RGB.} 
The majority of researches of adversarial attacks focus on RGB images, and the vulnerabilities of visual AI based on other spectral modalities are less explored. 
% A few existing related methods focus on attacking AI using thermal infrared images. 
Zhu~\etal~\cite{zhu2021fooling} proposed an adversarial attack method that creates thermal infrared patterns using glowing light bulbs. Later, they further designed an infrared invisible clothing using aerogel material to fool state-of-the-art human detectors~\cite{Zhu_2022_CVPR}. 
% However, the limitation of these methods are still obvious: the physical implementation of these methods (light bulbs, clothing with special material and patterns) are too attention-grabbing, which is contrary to the mission of adversarial attacks. 
For blackbox adversarial attack, HotCold Block~\cite{wei2022hotcold} was recently proposed to perform thermal infrared attack by using warming paste and cooling paste. 

To attack NIR face detection, Yamada~\etal~\cite{yamada2013privacy,yamada2012use} used electronic devices worn on the face that emit near-infrared lights to hide human faces from being identified. However, it is not wise to extend such an active method to hide full body from cameras. Our method is fully passive grounded on the physical characteristics of modern surveillance camera systems, and it attacks advanced human detectors. 
To our knowledge, no research has been conducted to disclose the vulnerability of NIR-based visual AI for human body detection, in spite of the fact that this is directly relevant to nighttime surveillance systems widely installed for daily usage. 
%In this paper, we explore adversarial attack on NIR-based human body detectors for the first time, and hope that this study will attract more attention on the trustworthiness of NIR-based AI.


\section{Vulnerabilities of NIR Photography}
\label{sec:vul}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/textureloss2.pdf}
\setlength{\abovecaptionskip}{-4mm}
\caption{Analysis on texture loss in NIR. (a) RGB images, (b) 850nm NIR images. (c) 50 spectral reflectance sampled from each scene. We can see that the spectral reflectances of different scene points tend to coincide around 850nm. }
\label{fig:textureloss2}
\vspace{-2mm}
\end{figure}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/textureloss2_SYS.pdf}
\setlength{\abovecaptionskip}{-3mm}
\caption{Examples of color and texture loss in human clothes from public datasets~\cite{wu2017rgb}.}
\label{fig:textureloss_SYS}
\vspace{-6mm}
\end{figure}



In this section, we analyze the fundamental vulnerabilities of NIR surveillance from three aspects: color loss, texture loss, and co-located settings. These three vulnerabilities allow our fully passive yet effective attack in both the digital world and the physical world, which will be further described in Sec.~\ref{sec:method}.

\noindent \textbf{Color loss.} For dual-mode surveillance cameras, NIR images are captured by trichromatic sensors with spectral sensitivities in the NIR range. However, different from RGB images, NIR images appear to be monochromatic. The fundamental reason is that the Camera Spectral Sensitivity (CSS) in the NIR range is almost the same for Red, Green, and Blue channels. As shown in Fig.~\ref{fig:colorloss}, the intensity of three channels coincide in the NIR range, leading to gray-scale output. As a result, the distribution of NIR images is simpler, with lower color variations compared to RGB images due to color loss. 

\noindent \textbf{Texture loss.} In addition to color loss, the texture loss further makes NIR data distribution more monotonic. Fig.~\ref{fig:textureloss} shows three types of images taken by the same color camera through different filters. We can see that the texture of cloth, dye, and fabrics gradually disappears in the NIR ranges ($>$ 700nm), and the texture loss becomes even worse when only using light around 850nm. The fundamental reason lies in the spectral reflectance of these materials. From Fig.~\ref{fig:textureloss2}, we can see that the spectral reflectance of different scene points varies a lot in the RGB range, but tends to be overlapped in the NIR range, especially around 850nm. Thus, these materials can produce different RGB observations but have almost the same appearance in an 850nm NIR image. 

Given the severe color and texture loss in 850nm NIR images, it is observed that clothes worn by people have rather simple distributions than RGB images -- uniform white with no texture. Fig.~\ref{fig:textureloss_SYS} shows some real-world examples from~\cite{wu2017rgb}. We argue that this makes AI models trained on such data less robust and can easily fail when encountering more complex or different data distributions.



\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{0mm}
\includegraphics[width=\linewidth]{pictures/pipeline.pdf}
\caption{Demonstration of one iteration for our pipeline. During each iteration, we update $N$ groups of binary patterns based on the detection results of the corresponding attacked images. The process involves sampling a batch of 3D human models and segmenting each of them into $K$ parts. We then generate 2D segmentation maps by rendering the models with arbitrary camera positions. Each part of the segment map is assigned a value of either $0$ or $255$ based on the corresponding binary pattern. We combine these maps with NIR backgrounds captured by a real camera system to generate the attacked NIR images. The detector then uses these images as input to produce the detection results. Finally, we update each binary pattern based on the detection results using selection and genetic operations.}
\label{fig:pipeline}
\vspace{-4mm}
\end{figure*}


\noindent \textbf{Co-located settings.} Given the simple and vulnerable distributions of 850nm NIR images, effective attacks can be achieved by manipulating the light distribution of NIR images. We notice that surveillance camera systems always have NIR LEDs mounted around the lens (Fig.~\ref{fig:colocated}), for the sake of saving installation space and avoiding occlusion. However, this co-located setting may easily lead to saturation and over-exposure when the direction of the light beam emitted from the LED matches the direction of the light beam entering the lens. Furthermore, if the camera’s auto-exposure function is activated to reduce the saturation effect, other image areas are likely to be darkened. 
Given these characteristics of NIR-based surveillance, we believe that it is possible to easily manipulate the local luminance distribution of images for an effective attack.




\section{Method}
\label{sec:method}
We first introduce how we control local light intensity for an effective attack using two types of tapes. We then introduce the composition of the designed adversarial attacker in the digital space and finally describe our proposed adversarial searching algorithm on how to find effective adversarial patterns.



\subsection{Problem Definition}

Given an NIR image $I \in \mathbb{R}^{3 \times H \times W}$ where $H$ and $W$ are respectively the height and width of the input image, the pre-trained human detector $F$ will return an output label $\mathcal{Y}$ that includes the position of the bounding boxes $Y_{pos}$, and the corresponding confidence $Y_{conf}$:
\begin{align}
    \mathcal{Y} = F(I) = [Y_{pos}, Y_{conf}].
\end{align}
Our goal is to fool the human detector and make it fail to detect humans in the images, \ie, minimizing the $Y_{conf}$:
\begin{align}
    \arg \min Y_{conf}.
\end{align}
To achieve this, we design an attack algorithm $f_{atk}$ that takes an NIR image $I$ as input and outputs the attacked image $\hat{I}$ for which the human detector has the lowest confidence:
\begin{align}
    \arg \min F(f_{atk}(I)).
\end{align}


\subsection{Manipulating Light Intensity with Tapes}


Using the feature of surveillance camera systems mentioned in Sec.~\ref{sec:vul}, we consider two types of tapes that can easily manipulate the local intensity of NIR images: Black plastic tapes (\eg, electrical insulating tape) have low NIR reflectance, enabling them to reduce the luminance value of an NIR image. Retro-reflective tapes, on the other hand, are made based on the retroreflective principle which can increase the luminance value because the direction of the light beam emitted from the LED and the direction of the light beam entering the lens are always the same, regardless of the orientation of the tape. By using these two types of tapes, we can easily control the local intensity of an NIR image to either black or white. Fig.~\ref{fig:tapes} show the performance of these tapes. We can see that the tapes can easily achieve light intensity manipulation due to their optical properties as long as the light and the camera are in co-located settings. Another observation is that the performance of retro-reflective tape is independent of its visible color, and even black retro-reflective tape can equally brighten NIR images, a key advantage that allows implementing physical attackers with natural and coherent appearances to human eyes. 





\subsection{Adversarial Medium Design in Digital Space}

\label{sec:digital}

In this section, we provide a detailed explanation of our adversarial medium design pipeline, which is illustrated in Fig.~\ref{fig:pipeline}. Our approach involves updating $N$ groups of binary patterns in each iteration, where the length of each pattern is $K$. To achieve this, we begin by obtaining 3D human models and partitioning each of them into $K$ parts. We then generate 2D segmentation maps by rendering these models from various camera positions. For each part of the segmentation map, we assign a value of either $0$ or $255$ based on the corresponding binary pattern. These maps are combined with actual NIR backgrounds captured by our camera system to create the attacked NIR images. The detector uses these images as input and produces detection results. We then utilize selection and genetic operations to update the binary patterns based on the detection results obtained for each pattern.



In the following paragraphs, we will introduce each part respectively, including 3D model segmentation and rendering, in-the-wild NIR image capture, adversarial pattern simulation, detection, binary pattern selection, and genetic operation. 


\subsubsection{3D model segmentation and rendering.} To perform the 3D physics-based adversarial attack, we need to mimic the real-world scenario in the digital space to assure that our result, searched in the digital space, can also generalize when adapting to the physical space. To achieve this, we adopt 3D models and rendering techniques to our pipeline. For 3D models, we use the most widely used SMPL-based~\cite{SMPL_2015,SMPL_X_2019,MANO_SIGGRAPHASIA_2017} human models, and randomly sample motions from the CMU Graphics Lab Motion Capture Database~\footnote{http://mocap.cs.cmu.edu/}. 






To generate 2D segmentation maps, we need to segment each of the 3D human models into $K$ pieces. The segmentation process is shown in Fig.~\ref{fig:segmentation}. We start from the standard SMPL~\cite{SMPL_2015,SMPL_X_2019,MANO_SIGGRAPHASIA_2017} human model which has 6890 vertices and split it into $K=31$ pieces according to the semantic meanings of each part. It is worth noting that meshes generated by the SMPL model have the same number of vertices, order, and connectivities, regardless of the 3D mesh's identity or motion. This consistency ensures that our 3D segmentation results remain uniform across various 3D models. Given that attaching tapes to the head, hands, and feet of a human body can be difficult, it is beneficial to attach NIR texture instead of either black or white to the corresponding parts (a total of 5 pieces) of the 3D model. However, there is currently no research or datasets available on 3D texture modeling for these parts in the NIR domain. Considering the auto-exposure function (disussed in Sec.~\ref{sec:vul}) that has been widely adapted to the nighttime surveillance systems, we provide two types of patterns: 1) forcing head, hands, and foots’ part to black (5black), and 2) forcing head to black (1black).


Finally, we randomly sample camera poses and render the 2D segmentation maps.





\subsubsection{Adversarial pattern simulation.}

As discussed in Sec.~\ref{sec:vul}, illumination intensities in the NIR images can be easily controlled by electrical insulating tape (low intensity, \ie, black) and retro-reflective tapes (high intensity, \ie, white). To create our adversarial pattern, we define the value of each pixel as a binary variable $x \in \{0,255\}$, with $0$ representing black and $255$ representing white. Based on the synthesized 2D segmentation maps, we assign each pixel in a given region of the map to either $0$ or $255$ based on $K$-length binary patterns that are updated during the searching process. We maintain $N$ binary patterns during the search, each of which produces a different adversarial pattern for attack, as illustrated in Fig.~\ref{fig:adversarial}.

\noindent \textbf{In-the-wild NIR background image.} Since the adversarial patterns can not simulate background contents in NIR images, we capture in-the-wild NIR images using the GS3-U3-15S5C camera with the 850nm band-pass filter to provide real NIR backgrounds for simulated attack images. For each group of adversarial patterns, we randomly sample NIR backgrounds during the search process.

\subsubsection{Detection.}

After obtained the simulated attacked NIR images $\hat{I} \in \mathbb{R}^{3 \times H \times W}$ where $H$ an $W$ are respectively the height and width of the image, we feed them into the pre-trained human detector $F$ and obtain the position of the bounding boxes $Y_{pos}$, and the corresponding confidence $Y_{conf}$:
\begin{align}
    F(\hat{I}) = [Y_{pos}, Y_{conf}].
\end{align}







\subsubsection{Binary pattern selection.}

Retrieving the optimal pattern without gradient from the target model is not an easy task. Here we search for the optimal adversarial pattern based on the Genetic Algorithm since our patterns are controlled by binary values. 

During each iteration, we select a portion of the existing binary patterns to reproduce for the next iteration. Each binary pattern is selected through a ranking-based process, where individuals with higher rankings (as measured by a ranking function) are more likely to be selected.

Since our goal is to fool the human detector and makes it fail to detect humans in the images, \ie, minimizing the $Y_{prob}$, we use the average confidence $c_i$ on the image batch to evaluate the fitness of each binary pattern. For each binary pattern, we calculate a ranking score $f_i$ through the ranking function:
\begin{align}
    f_i = \frac{c_{max}-c_i}{c_{max}-c_{min}},
\end{align}
where $c_{max}$ is the maximum value among all $c_i$, and $c_{min}$ is the minimum value.

These ranking scores are used to select better patterns to the next iteration. Specifically, each binary pattern has a chance of $p_i$ to be chosen for the next iteration, where $p_i$ is defined as:
\begin{align}
    p_{n}=\frac{f_n}{\sum_{j=0}^{N-1} f_j}.
\end{align}
Note that the selection process will be performed $N$ times to generate $N$ individuals for the next iteration.





\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{pictures/tapes.pdf}
\setlength{\abovecaptionskip}{2mm}
\caption{Performance of retro-reflective tape and insulating tape, when captured by a camera with co-located 850nm LED. Red: retro-reflective tape. Green: insulating tape. Blue: insulating tape pasted to a bigger retro-reflective tape. We can see that the retro-reflective tapes are always bright, irrespective of their visible colors.}
\label{fig:tapes}
\vspace{-4mm}
\end{figure}


\vspace{-4mm}



\begin{figure}[t]
\centering
\setlength{\abovecaptionskip}{-1mm}
\includegraphics[width=\linewidth]{pictures/segmentation.pdf}
\caption{Our segmentation paradigm on 3D human models to obtain 2D segmentation maps. Given the standard SMPL~\cite{SMPL_2015,SMPL_X_2019,MANO_SIGGRAPHASIA_2017} Human Body Model which has 6890 vertices, we segment all the vertices into 31 groups according to the semantic meanings of each part. Thanks to the homeomorphism characteristics of all meshes generatd by the SMPL-based model, the segmentation results remain consistent on different 3D models with different identities and motions. We then render these models with various camera extrinsics and obtain the 2D segmentation maps.}
\label{fig:segmentation}
\vspace{-4mm}
\end{figure}





\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{0mm}
\includegraphics[width=\linewidth]{pictures/adversarial.pdf}
\caption{Demonstration for the adversarial pattern synthesis. Given a batch of 2D segmentation maps rendered from various views, we assign values of $0$ or $255$ to each segment of the maps based on different binary patterns (assign $255$ when the binary pattern equals to $1$) to create the adversarial patterns. We then combine these adversarial patterns with real NIR backgrounds captured by our system to create the final attacked images. We feed these images to the detector and compute the average confidence score for each binary pattern, which we use to evaluate their rank in the subsequent selection process.}
\label{fig:adversarial}
\vspace{-2mm}
\end{figure*}






\subsubsection{Genetic operation.}

Once we have selected a portion of the binary patterns through the ranking-based process, we apply traditional Genetic Algorithm operations including Crossover and Mutation. The probability of Crossover and Mutation is determined by $P_{cross}$ and $P_{mut}$, respectively. In Crossover, we randomly select two binary patterns and determine a crossover index. The parts of these two binary patterns are then exchanged from the crossover index. For Mutation, we randomly choose a mutation index and change its value (either $0 \rightarrow 1$ or $1 \rightarrow 0$).





% \subsection{Blackbox Attack Optimization}
% Retrieving the optimal pattern without gradient from the target model is not an easy task. Based on the Genetic Algorithm, we optimize our adversarial medium given the image set $\mathcal{I}$ and the pre-trained detection model $f$. Fig.~\ref{fig:pipeline} shows the illustration for our optimization algorithm. 

% \noindent \textbf{Initialization.} To start with, we initialize $N$ individuals which respectively have two genetic properties standing for the position and shape of the adversarial medium. The position property include two binary vectors, each of which has a length of $L_{pos}$. The two vectors are corresponding to the normalized 2D spatial coordinate of the upper-left corner of the adversarial medium to the detected human bounding box. The shape property is a binary vector with a length of $L_{patt}$. Note that $L_{patt}$ is actually equal to the number of regions in the chosen pattern.

% \noindent \textbf{Add adversarial medium.} After initialization, we sample $B$ images from the image set $\mathcal{I}$, and add adversarial mediums to them. Specifically, we convert binary formulations to normalized spatial coordinates and binary patterns and add the adversarial mediums to the target region. For the position vector, we treat the vector as binary integers, then divide it with the maximum value given the length of $L_{pos}$:
% \begin{align}
%     a &= \frac{\operatorname{bin2int}(\mathcal{V}^{w}_{pos})}{2^{L_{pos}}},\\
%     b &= \frac{\operatorname{bin2int}(\mathcal{V}^{h}_{pos})}{2^{L_{pos}}},
% \end{align}
% where $\operatorname{bin2int}$ is the function to convert binary vectors to integers. For the pattern vector, we visit each element and assign white (1) or black (0) to the corresponding region according to the binary value. We then add the designed adversarial medium to each sampled image. 

% \noindent \textbf{Detection.} After adding the adversarial medium, we feed the image batch to the pre-trained detector to obtain the confidence score $Y_{prob}$. Note that we sample $B$ images for each batch and assign $N$ adversarial mediums for each image, so we will have a total of $B \times N$ attacked images for each iteration.

% \noindent \textbf{Selection.} During each iteration, we select a portion of the existing individuals to reproduce for the next iteration. Each individual is selected through a fitness-based process, where fitter individuals (as measured by a fitness function) are more likely to be selected. Specifically, we calculate the average confidence predicted by the detector on $B$ images for each individual and calculate the fitness for it as:
% \begin{align}
%     f_n = \frac{c_{max} - c_n}{c_{max} - c_{min}},
% \end{align}
% where $f_i$ is the fitness of the $i$-th individual, and $c_n$ si the average confidence on $B$ images for the $i$-th individual. $c_{max}$ and $c_{min}$ stand for the maximum and minimum average confidence among all individuals, respectively. Based on the fitness $f_i$, each individual has a chance of $p_i$ to be chosen for the next iteration, where $p_i$ is defined as:
% \begin{align}
%     p_{n}=\frac{f_n}{\sum_{j=0}^{N-1} f_j}.
% \end{align}
% Note that this selection process will be performed $N$ times to generate $N$ individuals for the next iteration.


% \noindent \textbf{Genetic operation.} We just use traditional Crossover and Mutation as our Genetic operation. The probability of Crossover and Mutation are respectively set to $P_{cross}$ and $P_{mut}$.



\section{Experiments}


% \begin{figure}[t]
% \centering
% % \setlength{\abovecaptionskip}{1mm}
% \includegraphics[width=\linewidth]{pictures/digital.pdf}
% \caption{Qualitative results of different adversarial patterns on digital space.}
% \label{fig:digital}
% % \vspace{-4mm}
% \end{figure}


\subsection{Settings}

% \noindent \textbf{Metrics.} We adopt two metrics to evaluate the effectiveness of our model: (1) Average Confidence (AC) for person class, which is defined as the average confidence the network outputed for the person class. (2) Attack Success Rate (ASR) ($\%$), which is defined as the percentage of positive and total samples as follows:
% \begin{align}
% \operatorname{ASR}=1-\frac{1}{N} \sum_{i=0}^{N} \operatorname{sign}(\text {label}_{i}) \\
% \operatorname{sign}(\text{label}_{i})=\left\{\begin{array}{l}
% 1, \ \text{label}_{i} \in L_{pre} \\
% 0, \ \text{otherwise.}
% \end{array}\right.
% \end{align}
% where $N$ is the number of all true positive labels detected in our dataset when there is no attack, $L_{pre}$ is the set of person labels detected under attacking. The higher the ASR, the more effective the adversarial attack method is.



\noindent \textbf{Metrics.} We adopt two metrics to evaluate the effectiveness of our model: (1) Average Confidence (AC) for person class, which is defined as the average confidence the detector outputted for the person class. (2) Attack Success Rate (ASR) ($\%$), which is defined as follows:
\begin{align}
\operatorname{ASR} = 1 - \frac{N_a}{N_0}
\end{align}
where $N_0$ is the number of all true positive labels detected in our dataset when there is no attack, and $N_a$ is the number of all person labels detected in our dataset after attack. The higher the ASR, the more effective the adversarial attack method is.

\noindent \textbf{Implementation details.} 
We use YOLOv5~\footnote{https://github.com/ultralytics/yolov5} as our target model since it is fast, effective, and widely used. We first use YOLO5S with the official checkpoint as our attack target. We then finetune an NIR version of YOLO5S on our collected NIR dataset and use it as our attack target. Our collected dataset to finetune YOLO5S contains 13000 video frames of 13 identities with varying and cluttered backgrounds, and each identity has 500 frames of frontside and 500 frames of backside. During the searching process, the number of binary patterns is set to $N=1000$, and the image batch size is set to $B=300$. $P_{cross}$ and $P_{mut}$ are set to 0.5 and 0.01, respectively. We conduct all experiments on an NVIDIA GeForce RTX 3090 GPU, and all our codes are implemented in PyTorch~\cite{paszke2019pytorch}.

\noindent \textbf{Details of Digital Data Synthesis.} As has been mentioned in Sec.~\ref{sec:digital}, to perform pattern search and attack in digital space, we incorporate SMPL and CMU Graphics Lab Motion Capture Database to synthesize different 3D human meshes and introduce different motions to generate our human model, then segment and render these 3D meshes with different camera extrinsics. We then add random backgrounds from our taken real NIR images. To achieve this, we randomly generate 428 human meshes with different identities and motions, then segment and render each human model with 25 different camera extrinsics. These lead to 10700 different 2D segment maps. We use 8560 of them to search the adversarial pattern via our proposed algorithm and use the rest 2140 to test the effectiveness of our designed adversarial pattern. The random NIR backgrounds come from 909 NIR images taken at nighttime with camera GS3-U3-15S5C and two co-located 850nm NIR LEDs.



\begin{table}[!t]
\centering
% \setlength{\abovecaptionskip}{1mm}
\caption{Average Confidence (AC) and Attack Success Rate (ASR) ($\%$) results of different adversarial patterns on digital space. Best results are in \textbf{Bold}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{Patterns} & \multicolumn{2}{c}{Finetuned YOLO} & \multicolumn{2}{c}{Official YOLO}                           \\
\cmidrule(r){2-3} \cmidrule(r){4-5}
      & AC $\downarrow$ & ASR $\uparrow$ & AC $\downarrow$ & ASR $\uparrow$ \\ 
\midrule
All black     & 0.182 $\pm$ 0.002 & 75.94 $\pm$ 0.68 & 0.853 $\pm$ 0.001 & 0.72 $\pm$ 0.18 \\
All white     & 0.262 $\pm$ 0.003 & 58.41 $\pm$ 0.57 & 0.567 $\pm$ 0.004 & 23.23 $\pm$ 0.58 \\
Random        & 0.160 $\pm$ 0.030 & 79.80 $\pm$ 6.88 & 0.655 $\pm$ 0.083 & 12.88 $\pm$ 7.99 \\
Ours (5black)          & 0.098 $\pm$ 0.002 & 93.44 $\pm$ 0.49 & 0.370 $\pm$ 0.004 & 46.64 $\pm$ 0.84 \\
Ours (1black)          & \textbf{0.097 $\pm$ 0.001} & \textbf{94.14 $\pm$ 0.45} & \textbf{0.301 $\pm$ 0.004} & \textbf{56.23 $\pm$ 1.11} \\

\bottomrule
\end{tabular}
}
\label{tab:digital}
% \vspace{-2mm}
\end{table}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/digital.pdf}
\setlength{\abovecaptionskip}{-2mm}
\caption{Qualitative attack results of different patterns on the Official YOLO in the digital space. Images are cropped for visualization.}
\label{fig:digital}
\vspace{-4mm}
\end{figure}




\subsection{Results}



\subsubsection{Digital Attack.}

We compare five types of attack patterns based on the binary intensity manipulation, including 1) letting all body parts be black (All black), 2) letting all body parts be white except for the head (All white), 3) random assigning $0$ or $1$ to each body part, 4) using our algorithm to search the adversarial patterns with head, hands, and foots' part set to black (Ours, 5black), and 5) using our algorithm to search the adversarial patterns with head part set to black (Ours, 1black). The quantitative and qualitative results for digital attack are shown in Tab.~\ref{tab:digital} and Fig.~\ref{fig:digital}, respectively. We can see that the adversarial patterns designed by our algorithm have the best attack performance on two types of YOLO5 (Official checkpoint and finetuned checkpoint) in terms of both Average Confidence (AC) and Attack Success Rate (ASR). We can also see that after being finetuned on NIR datasets, the YOLO model is easier to attack and becomes less robust to the adversarial patterns. This verifies the severe vulnerabilities of a visual AI algorithm trained on NIR images with limited variation, as analyzed in Sec.\ref{sec:vul}. 


\subsubsection{Physical Attack.}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/physical_3.pdf}
\setlength{\abovecaptionskip}{-2mm}
\caption{Qualitative results of our designed pattern in the physical space. Images are cropped for visualization.}
\label{fig:physical}
\vspace{-4mm}
\end{figure}


To further justify the effectiveness of our proposed attack method, we physically realize our adversarial patterns in the physical space by using the retro-reflective tapes (\ie, white) and the electrical insulating tapes (\ie, black), and use them to attack the official YOLO. During the physical attack process, we take pictures from 360 degrees of the human body and various distances to justify the effectiveness of our 3D-aware design pipeline. Specifically, we perform two groups of experiments: 1) We respectively take pictures from various angles and distances of one person with no adversarial pattern, all-white adversarial patterns, and our designed adversarial patterns. 2) We simultaneously take pictures of groups of persons with different adversarial patterns using the same camera, including one person with no adversarial pattern, one person with the all-white adversarial patterns, and one person with our designed adversarial patterns. While being captured, each person displays distinct actions instead of remaining stationary. The results are reported in Tab.~\ref{tab:physical}, Fig.~\ref{fig:physical}, and Fig.~\ref{fig:physical_compare}.

From Tab.~\ref{tab:physical}, we can see that our designed patterns achieve significant attack performances in the physical space, with an average Average Confidence (AC) of 0.088 and an average Attack Success Rate (ASR) of 87.93\%. Corresponding qualitative results are shown in Fig.~\ref{fig:physical}. We also analyze the impact of distances on the physical attack by collecting adversarial samples of different distances. We can see that both AC and ASR become worse as the distance of the person becomes closer to the camera. The reasons are two folds: 1) the pixel values of electrical insulating tapes no longer remain 0 when the distance becomes too close, corrupting the adversarial patterns. 2) the human head, hands and feet becomes more visible when the distance becomes very close. Considering the fact that surveillance cameras are typically installed at a considerable distance from the monitored area, we can infer that our model is relevant and meaningful for practical surveillance scenarios.



\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/physical_compare.pdf}
\setlength{\abovecaptionskip}{-2mm}
\caption{Qualitative comparisons between our designed patterns, all-white patterns, and no adversarial pattern in the physical space. (a) Our designed patterns and all-white patterns, (b) Our designed patterns and no adversarial pattern. Images are cropped for visualization.}
\label{fig:physical_compare}
\vspace{-3mm}
\end{figure}


\begin{table}[!t]
\centering
\setlength{\abovecaptionskip}{2mm}
\caption{Average Confidence (AC) and Attack Success Rate (ASR) ($\%$) results of different distances in physical space. For ``No Attack'', we use Detection Rate (DR) instead of ASR. Best results are in \textbf{Bold}.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Distance} & \multicolumn{2}{c}{No attack} & \multicolumn{2}{c}{All white} & \multicolumn{2}{c}{Ours} \\
\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7}
      & AC & DR & AC $\downarrow$ & ASR $\uparrow$ & AC $\downarrow$ & ASR $\uparrow$ \\ 
\midrule
% 2m     & 0.914 & 100.0 & 0.217 & 65.52 & \textbf{0.294} & \textbf{43.95} \\
3m     & 0.888 & 100.0 & 0.411 & 32.64 & \textbf{0.152} & \textbf{76.22} \\
4m     & 0.827 & 98.78 & 0.373 & 33.65 & \textbf{0.075} & \textbf{91.20} \\
5m     & 0.715 & 96.30 & 0.439 & 28.27 & \textbf{0.038} & \textbf{96.36} \\
\midrule
Average     & 0.810 & 98.36 & 0.408 & 31.52 & \textbf{0.088} & \textbf{87.93} \\
\bottomrule
\end{tabular}
}
\label{tab:physical}
\vspace{-4mm}
\end{table}


Fig.~\ref{fig:physical_compare} further shows the comparison between different patterns. We can see that the detector successfully detects the person without the adversarial patterns in the picture, but fail to detect the person with our designed adversarial patterns. We can also see that our designed patterns are more effective than all-white patterns in attacking the detector, which can also be verified by Tab.~\ref{tab:physical}.



% \begin{figure}[t]
% \centering
% \includegraphics[width=\linewidth]{pictures/tapesrgb.jpeg}
% % \setlength{\abovecaptionskip}{-2mm}
% \caption{.}
% \label{fig:st}
% % \vspace{-4mm}
% \end{figure}



\subsubsection{Evaluation of stealthiness.} 
We choose retro-reflective tapes and electrical insulating tapes as our adversarial medium. One extra benefit is that the performance of these tapes is independent of their visible color, and even black retro-reflective tape can equally brighten NIR images, allowing the implementation of physical attackers with a natural and coherent appearance to human eyes. As shown in Fig.~\ref{fig:stealthiness}, it is clear that the adversarial mediums are in harmony with clothes and do not draw attention, especially in night environment.

\section{Discussions}


\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{pictures/stealthiness.pdf}
\setlength{\abovecaptionskip}{-2mm}
\caption{Examples of RGB-NIR images with adversarial patterns. (a) RGB image under normal light, (b) RGB image under low light, (c) NIR image under co-located 850nm LED.}
\label{fig:stealthiness}
\vspace{-6mm}
\end{figure}

\noindent \textbf{Research ethics.}
In line with existing researches on adversarial attacks, our motivation for this study is to arouse due attention to the reliability of NIR-based AI, which has been deployed in commercial surveillance systems. We hope countermeasures to detect such attacks, through data filtering, enhancement, and more complicated strategies, could be proposed for better reliability.%. 

\noindent \textbf{Defense methods.}
By fine-tuning the detectors on datasets containing our adversarial patterns, they are expected to become more robust against our attack. Additionally, another fundamental defense strategy involves altering the co-located setting of the surveillance system. 
Without the co-located setting, our tapes would fail to produce 'white' adversarial patterns, resulting in unsuccessful attacks. However, changing the co-located setting introduces various challenges, including occlusion and increased space occupation.

\noindent \textbf{Limitations and future works.}
Although our work achieves significant attack performances in both digital and physical space, our model cannot faithfully model the head, hands, and feet texture of human bodies in the NIR domain, which leads to failure cases at very near distances. In future work, we aim to resolve this problem by collecting NIR human skin texture for more realistic rendering. 

\vspace{-1mm}
\section{Conclusion}
In this paper, we have revealed the fundamental vulnerabilities of NIR-based AI that are widely deployed in surveillance camera systems for daily use. Due to the characteristics of the spectral response of silicon sensors and the reflectance of dyed clothing, images captured in the NIR range suffer from color loss and texture loss. The special geometric configuration of the illuminant and the camera in a nearly co-located setup further allows manipulation of image intensity easily in the physical world, by using retro-reflective tapes and insulating tapes. We showed the success of attacking a YOLO-based human detector by designing an adversarial attacker in the digital space using 3D-aware techniques and later implementing it in the physical world, which arouses concerns about the reliability of surveillance systems powered by NIR-related AI algorithms.

\vspace{-1mm}
\section*{Acknowledgements}
This work was partially supported by JSPS KAKENHI Grants 21H04907, 22H00529, 20H05951, JST CREST Grants JPMJCR18A6, JPMJCR20D3, and ROIS NII Open Collaborative Research 2023-23S1201. 

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{sample-base}


\end{document}
\endinput
%%
%% End of file `sample-sigconf.tex'.

